Search for top squark pair production in final states with one isolated lepton, jets, and missing transverse momentum in $\sqrt{s}=$ 8 TeV pp collisions with the ATLAS detector

The results of a search for top squark (stop) pair production in final states with one isolated lepton, jets, and missing transverse momentum are reported. The analysis is performed with proton--proton collision data at $\sqrt{s} = 8$ TeV collected with the ATLAS detector at the LHC in 2012 corresponding to an integrated luminosity of $20$ fb$^{-1}$. The lightest supersymmetric particle (LSP) is taken to be the lightest neutralino which only interacts weakly and is assumed to be stable. The stop decay modes considered are those to a top quark and the LSP as well as to a bottom quark and the lightest chargino, where the chargino decays to the LSP by emitting a $W$ boson. A wide range of scenarios with different mass splittings between the stop, the lightest neutralino and the lightest chargino are considered, including cases where the $W$ bosons or the top quarks are off-shell. Decay modes involving the heavier charginos and neutralinos are addressed using a set of phenomenological models of supersymmetry. No significant excess over the Standard Model prediction is observed. A stop with a mass between $210$ and $640$ GeV decaying directly to a top quark and a massless LSP is excluded at $95$ % confidence level, and in models where the mass of the lightest chargino is twice that of the LSP, stops are excluded at $95$ % confidence level up to a mass of $500$ GeV for an LSP mass in the range of $100$ to $150$ GeV. Stringent exclusion limits are also derived for all other stop decay modes considered, and model-independent upper limits are set on the visible cross-section for processes beyond the Standard Model.

==> boostedsymbols.tex <==
\RequirePackage{xspace}

\newcommand{\Rmin}       {\ensuremath{R_{\rm min}}}
\newcommand{\DeltaR}     {\ensuremath{\Delta R}}
\newcommand{\DetaDphi}   {\ensuremath{\sqrt{(\Delta \eta)^{2} + (\Delta\phi)^{2}}}\xspace}
\newcommand{\DyDphi}     {\ensuremath{\sqrt{(\Delta y)^{2} + (\Delta\phi)^{2}}}\xspace}
\newcommand{\DeltaRdef}  {\ensuremath{\DeltaR = \DetaDphi}\xspace}
\newcommand{\DeltaRydef} {\ensuremath{\DeltaR = \DyDphi}\xspace}
\newcommand{\DeltaRtrk}  {\ensuremath{\Delta R({\rm trk}_1,{\rm trk}_2)}}
\newcommand{\ptjet}  {\ensuremath{\pt^\mathrm{jet}}}

\newcommand{\mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\mlead}     {\ensuremath{\mjet_{1}}\xspace}
\newcommand{\mleadavg}  {\ensuremath{\langle\mlead\rangle}\xspace}
\newcommand{\Mjet}      {\mjet}
\newcommand{\massjet}   {\mjet}
\newcommand{\mThresh}   {\ensuremath{M_{\rm threshold}}\xspace}
\newcommand{\mjetAvg}   {\ensuremath{\langle\mjet\rangle}\xspace}
\newcommand{\masstrkjet}{\ensuremath{m^{\rm track \; jet}}\xspace}

\newcommand{\Wmass}     {\ensuremath{m_{\Wboson}}\xspace}
\newcommand{\WmassT}    {\ensuremath{m^{\Wboson}_{T}}\xspace}
\newcommand{\topmass}   {\ensuremath{m_{\rm top}}\xspace}
\newcommand{\massZprime}{\ensuremath{m_{\Zprime}}\xspace}

\newcommand{\antikt}{anti-$k_{t}$}
\newcommand{\akt}       {\antikt\xspace}
\newcommand{\Akt}       {\Antikt\xspace}
\newcommand{\AKT}       {\akt}
\newcommand{\AKTFat}    {\antikt, \ensuremath{R=1.0}\xspace}
\newcommand{\AKTPrune}  {\antikt, \ensuremath{R=1.0} (pruned)\xspace}
\newcommand{\AKTFilt}   {\antikt, \ensuremath{R=1.0} (filtered)\xspace}
\newcommand{\KTSix}     {\ensuremath{k_{t}}, \ensuremath{R=0.6}\xspace}
\newcommand{\kt}        {\ensuremath{k_{t}}\xspace}
\newcommand{\ca}        {Cambridge-Aachen\xspace}
\newcommand{\CamKt}     {\ensuremath{\mathrm{C/A}}\xspace}
\newcommand{\CASix}     {\CamKt, \ensuremath{R=0.6}\xspace}
\newcommand{\CAFat}     {\CamKt, \ensuremath{R=1.2}\xspace}
\newcommand{\CAPrune}   {\CamKt, \ensuremath{R=1.2} (pruned)\xspace}
\newcommand{\CAFilt}    {\CamKt, \ensuremath{R=1.2} (filtered)\xspace}
\newcommand{\SISCone}   {SISCone}
\newcommand{\SISConeSiz}{\SISCone, \ensuremath{R=0.6}\xspace}
\newcommand{\minKt}     {\ensuremath{\min\left(\pti^2, \ptj^2\right)}\xspace}
\newcommand{\minAKt}    {\ensuremath{\min\left(\pti^{-2}, \ptj^{-2}\right)}\xspace}
\newcommand{\minGen}    {\ensuremath{\min\left(\pti^{2p}, \ptj^{2p}\right)}\xspace}
\newcommand{\Rij}       {\ensuremath{R_{ij}}\xspace}
\newcommand{\DRij}      {\ensuremath{\Delta\Rij}\xspace}
\newcommand{\DRratio}   {\ensuremath{\frac{\DRij^2}{R^2}}\xspace}
\newcommand{\diB}       {\ensuremath{d_{iB}}\xspace}
\newcommand{\Rfilt}     {\ensuremath{R_{\rm filt}}\xspace}
\newcommand{\jone}      {\ensuremath{J_{1}}\xspace}
\newcommand{\jtwo}      {\ensuremath{J_{2}}\xspace}
\newcommand{\sjone}     {\ensuremath{j_{1}}\xspace}
\newcommand{\sjtwo}     {\ensuremath{j_{2}}\xspace}
\newcommand{\msubjone}  {\ensuremath{m^{\sjone}}\xspace}
\newcommand{\msubjtwo}  {\ensuremath{m^{\sjtwo}}\xspace}
\newcommand{\mjone}     {\ensuremath{m^{\jone}}\xspace}
\newcommand{\mjtwo}     {\ensuremath{m^{\jtwo}}\xspace}
\newcommand{\ptsubjone} {\ensuremath{p_{T}^{\sjone}}\xspace}
\newcommand{\ptsubjtwo} {\ensuremath{p_{T}^{\sjtwo}}\xspace}
\newcommand{\Rsubjets}  {\ensuremath{R_{\sjone,\sjtwo}}\xspace}
\newcommand{\DRsubjets} {\ensuremath{\Delta\Rsubjets}\xspace}
\newcommand{\pti}       {\ensuremath{p_{{\rm T}i}}\xspace}
\newcommand{\ptj}       {\ensuremath{p_{Tj}}\xspace}
\newcommand{\ycut}      {\ensuremath{y_{\rm cut}}\xspace}
\newcommand{\mcut}      {\ensuremath{m_{\rm cut}}\xspace}
\newcommand{\ymin}      {\ensuremath{y_{\min}}\xspace}
\newcommand{\fcut}      {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}      {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\Nsubjet}      {\ensuremath{N_{\rm subjets}}\xspace}
\newcommand{\drsub}     {\ensuremath{\Rsub}\xspace}
\newcommand{\mufrac}    {\ensuremath{\mu_{\rm frac}}\xspace}
\newcommand{\rcut}      {\ensuremath{R_{\rm cut}}\xspace}
\newcommand{\zcut}      {\ensuremath{z_{\rm cut}}\xspace}
\newcommand{\largeR}    {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}    {Large-\ensuremath{R}\xspace}
\newcommand{\NjetStd}   {\ensuremath{N_{\rm jet}^{R4}}\xspace}

\newcommand{\ptrecojet}  {\ensuremath{\pt^\mathrm{reco \; jet}}}
\newcommand{\pttruejet}  {\ensuremath{\pt^\mathrm{truth \; jet}}}
\newcommand{\mrecojet}  {\ensuremath{m^\mathrm{reco \; jet}}}
\newcommand{\mtruejet}  {\ensuremath{m^\mathrm{truth \; jet}}}
\newcommand{\rjet}       {\ensuremath{r}\xspace}
\newcommand{\rjetPt}     {\ensuremath{\rjet^{p_T}}\xspace}
\newcommand{\rjetM}      {\ensuremath{\rjet^{m}}\xspace}

\newcommand{\rtrkjet}       {\ensuremath{r_{\rm track \; jet}}\xspace}
\newcommand{\rtrkjetPt}     {\ensuremath{\rtrkjet^{p_T}}\xspace}
\newcommand{\rtrkjetM}      {\ensuremath{\rtrkjet^{M}}\xspace}
\newcommand{\rtrkjetPtData} {\ensuremath{\rtrkjet^{p_{T},{\rm data}}}\xspace}
\newcommand{\rtrkjetMData}  {\ensuremath{\rtrkjet^{M,{\rm data}}}\xspace}
\newcommand{\rtrkjetPtMC}   {\ensuremath{\rtrkjet^{p_{T},{\rm MC}}}\xspace}
\newcommand{\rtrkjetMMC}    {\ensuremath{\rtrkjet^{M,{\rm MC}}}\xspace}
\newcommand{\RtrkjetPt}     {\ensuremath{R_{r{\rm \; track \; jet}}^{p_T}}\xspace}
\newcommand{\RtrkjetM}      {\ensuremath{R_{r{\rm \; track \; jet}}^{M}}\xspace}

\newcommand{\subjetpt}  {\ensuremath{p_{T}^{\rm subjet}}\xspace}
\newcommand{\yij}       {\ensuremath{y_{ij}}\xspace}
\newcommand{\dcut}      {\ensuremath{d_{\rm cut}}\xspace}
\newcommand{\dmin}      {\ensuremath{d_{\min}}\xspace}
\newcommand{\dij}       {\ensuremath{d_{ij}}\xspace}
\newcommand{\Dij}       {\ensuremath{\sqrt{\dij}}\xspace}
\newcommand{\DOneTwo}   {\ensuremath{\sqrt{d_{12}}}\xspace}
\newcommand{\DTwoThr}   {\ensuremath{\sqrt{d_{23}}}\xspace}
\newcommand{\yOneTwo}   {\ensuremath{y_{1}}\xspace}
\newcommand{\yTwoThr}   {\ensuremath{y_{2}}\xspace}
\newcommand{\yOneTwoDef}{\ensuremath{\yOneTwo=\DOneTwo/\mjet}\xspace}
\newcommand{\yTwoThrDef}{\ensuremath{\yTwoThr=\DTwoThr/\mjet}\xspace}
\newcommand{\xj}        {\ensuremath{x_{J}}\xspace}
\newcommand{\jetFunc}   {\ensuremath{J^{(eik),c} (\mjet,\pT,R)}\xspace}
\newcommand{\tauN}      {\ensuremath{\tau_N}\xspace}
\newcommand{\tauTwoOne} {\ensuremath{\tau_{21}}\xspace}
\newcommand{\tauThrTwo} {\ensuremath{\tau_{32}}\xspace}
\newcommand{\dip}       {\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dipOneTwo} {\ensuremath{\dip_{12}}\xspace}
\newcommand{\dipTwoThr} {\ensuremath{\dip_{23}}\xspace}
\newcommand{\dipOneThr} {\ensuremath{\dip_{13}}\xspace}

\newcommand{\Zprimett}  {\ensuremath{\Zprime\ra t\bar{t}}\xspace}
\newcommand{\Zqq}       {\ensuremath{Z\ra q\bar{q}}\xspace}
\newcommand{\Wqq}       {\ensuremath{W\ra q\bar{q}}\xspace}

\newcommand{\mpi}{multiple parton interactions\xspace}

